The Ontological Key: Automatically Understanding and Integrating Forms to Access the Deep Web

Forms are our gates to the web. They enable us to access the deep content of web sites. Automatic form understanding provides applications, ranging from crawlers over meta-search engines to service integrators, with a key to this content. Yet, it has received little attention other than as component in specific applications such as crawlers or meta-search engines. No comprehensive approach to form understanding exists, let alone one that produces rich models for semantic services or integration with linked open data. In this paper, we present OPAL, the first comprehensive approach to form understanding and integration. We identify form labeling and form interpretation as the two main tasks involved in form understanding. On both problems OPAL pushes the state of the art: For form labeling, it combines features from the text, structure, and visual rendering of a web page. In extensive experiments on the ICQ and TEL-8 benchmarks and a set of 200 modern web forms OPAL outperforms previous approaches for form labeling by a significant margin. For form interpretation, OPAL uses a schema (or ontology) of forms in a given domain. Thanks to this domain schema, it is able to produce nearly perfect (more than 97 percent accuracy in the evaluation domains) form interpretations. Yet, the effort to produce a domain schema is very low, as we provide a Datalog-based template language that eases the specification of such schemata and a methodology for deriving a domain schema largely automatically from an existing domain ontology. We demonstrate the value of the form interpretations in OPAL through a light-weight form integration system that successfully translates and distributes master queries to hundreds of forms with no error, yet is implemented with only a handful translation rules.

==> Makefile <==

# $Id: Makefile 27435 2012-02-17 12:50:28Z christian $ 

# This makefile builds a number of latex documents sharing the same
# dependencies.
#
# Thus, this makefile is intended either for 
#   * a large document with multiple main-files (e.g. with and without
#     comments), or
#   * a set of simple documents sharing some filees (e.g. macros)
#
# If PDFLATEX is set (to pdflatex), then pdf files are built without
# intermediate postscript files. 
#
#
# The MAIN FILES for all documents are in $tex_files, which defaults
# to the *.tex files in the working directory.
#
# The DEPENDENCIES are taken recursively from 
#   * the paths in $include_path for *.tex, *.dia, *.gnuplot, and *.pdf files
#   * the current working directory for *.bib, *.cls, *.sty, and *.bst
#     files
#   * extra files of these types specified manually
#
# If any of these dependencies changes, all documents from $tex_files
# are to be rebuilt. The latex BUILD first  
#   * converts dia into eps files
#   * runs the gnuplot scripts to obtain pdfs
# and then executes
#   * latex once
#   * bibtex (if a .bbl file has been included)
#   * makeindex (if an index file has been included)
#   * latex once
#   * latex two more times, until cross references are stable
#
#
#
# The makefile offers GOALS for all documents in $tex_files:
#   * .dvi, .ps, .pdf as usual
#   * .embedded.pdf builds a pdf with all fonts embedded (relies on
#     $papersize)
#
# And it offers the following SUMMARY GOALS:
#   * allps, allpdf, all (usually same as allpdf), clean


################################################################################
#
# configuration
#
################################################################################

# The main tex file of the project
# (multiple files allowed---they all share the same dependencies)
tex_files=$(shell ls *.tex)

# include paths for tex and figures
include_path=include figures diadem

# extra bibtex files NOT found recursively in the root directory
bibtex_files=

# extra include files NOT found recursively in the include directories
tex_include_files=
gnuplot_include_files=
dia_include_files=
pdf_include_files=

# extra source files which are NEITHER tex, bib, dia, gnuplot,
# sty, bst, not cls
extra_source_files=

# extra clean files which are NOT caused by tex, dia, or gnuplot files
extra_clean_files=

# papersize for embedded pdf generation
papersize=a4


LATEX=latex
PDFLATEX=pdflatex # -interaction=nonstopmode
GNUPLOT_EXISTS=$(shell which gnuplot > /dev/null && echo 1)

################################################################################
#
# tex, fig, dia, pdf, gnuplot from $include_path
# sty, cls, bst, bib from .
#
################################################################################

# drop the directories which do not exist
include_path_filtered=$(wildcard $(include_path))

extra_source_files+= $(shell find . -name "*.sty")
extra_source_files+= $(shell find . -name "*.cls")
extra_source_files+= $(shell find . -name "*.bst")

bibtex_files+=$(shell find . -name "*.bib")

ifneq ($(include_path_filtered),)
tex_include_files+=$(shell find $(include_path_filtered) -name "*.tex")
ifeq ($(GNUPLOT_EXISTS),1)
gnuplot_include_files+=$(shell find $(include_path_filtered) -name "*.gnuplot")
endif
dia_include_files+=$(shell find $(include_path_filtered) -name "*.dia")
pdf_include_files+=$(shell find $(include_path_filtered) -name "*.pdf")
endif

################################################################################
#
# derived variables
#
################################################################################

source_files+=$(bibtex_files)

clean_files=$(tex_files:.tex=.bbl) \
            $(tex_files:.tex=.blg) \
            $(tex_files:.tex=.dvi) \
            $(tex_files:.tex=.log) \
            $(tex_files:.tex=.aux) \
            $(tex_files:.tex=.ps)  \
            $(tex_files:.tex=.pdf) \
            $(tex_files:.tex=.sdx) \
            $(tex_files:.tex=.toc) \
            $(tex_files:.tex=.ilg) \
            $(tex_files:.tex=.ind) \
            $(tex_files:.tex=.idx) \
            $(tex_files:.tex=.lot) \
            $(tex_files:.tex=.lof) \
            $(tex_files:.tex=.svn)

clean_files+=$(fig_include_files:.fig=.fig.tex) \
			 $(fig_include_files:.fig=.fig.log) \
			 $(fig_include_files:.fig=.fig.aux) \
			 $(fig_include_files:.fig=.fig.dvi) \
			 $(fig_include_files:.fig=.fig.eps) \
			 $(fig_include_files:.fig=.fig.pstex_t) \
			 $(fig_include_files:.fig=.fig.pstex) 


# dia to eps
dia_pdf_include_files+=$(dia_include_files:.dia=.pdf)
source_files+=$(dia_pdf_include_files)
clean_files+=$(dia_pdf_include_files)

# gnuplot to pdf
gnuplot_pdf_include_files=$(gnuplot_include_files:.gnuplot=.pdf)
pdf_include_files-=$(gnuplot_pdf_include_files)
gnuplot_ps_include_files=$(gnuplot_include_files:.gnuplot=.ps)
source_files+=$(gnuplot_pdf_include_files)
clean_files+=$(gnuplot_pdf_include_files)
clean_files+=$(gnuplot_ps_include_files)

# included tex files
source_files+=$(tex_include_files)
clean_files+=$(tex_include_files:.tex=.aux)

# pdfs 
source_files+=$(pdf_include_files)

# extra include
source_files+=$(extra_source_files)
clean_files+=$(extra_clean_files)

################################################################################
#
# rules (customize)
#
################################################################################

all: allpdf

.PHONY: allps allpdf	
allps: $(tex_files:.tex=.ps) 
allpdf: $(tex_files:.tex=.pdf)


################################################################################
#
# generic rules (do not change)
#
################################################################################

clean:
	rm -f $(clean_files)

# tex -> dvi ###################################################################

latex_needs_rerun_pattern="(There were undefined references|LaTeX Warning: Citation|Rerun to get (cross-references|the bars) right)"
latex_error_report_pattern="(There were undefined references|Rerun to get (cross-references|the bars) right)|undefined|Undefined|Missing|multiply-defined| multiply defined"

%.dvi: %.tex $(source_files)
	@echo
	@echo ">>>>>>>>>>> latexing $(@:.dvi=)  <<<<<<<<<<<"
	@$(LATEX) $(@:.dvi=) </dev/null
	@echo ">>>>>>>>>>> bibtexing $(@:.dvi=) <<<<<<<<<<<"
	@egrep "$(@:.dvi=.bbl)" $(@:.dvi=.log) >/dev/null && bibtex $(@:.dvi=) ; true
	@echo ">>>>>>>>>>> indexing $(@:.dvi=)  <<<<<<<<<<<"
	@egrep "Writing index file" $(@:.dvi=.log) | colrm 1 19 | xargs -n 1 makeindex ; true
	@echo ">>>>>>>>>>> latexing $(@:.dvi=)  <<<<<<<<<<<"
	@$(LATEX) $(@:.dvi=) </dev/null
	@egrep $(latex_needs_rerun_pattern) $(@:.dvi=.log) && \
     echo ">>>>>>>>>>> latexing $(@:.dvi=)  <<<<<<<<<<<" && $(LATEX) $(@:.dvi=) </dev/null; true
	@egrep $(latex_needs_rerun_pattern) $(@:.dvi=.log) && \
     echo ">>>>>>>>>>> latexing $(@:.dvi=)  <<<<<<<<<<<" && $(LATEX) $(@:.dvi=) </dev/null; true 
	@echo ">>>>>>>>>>> grepped error messages begin: $(@:.dvi=) <<<<<<<<<<<"
	@egrep $(latex_error_report_pattern) $(@:.dvi=.log) | grep -v "Missing character:" ; true
	@echo ">>>>>>>>>>> grepped error messages end: $(@:.dvi=) <<<<<<<<<<<"


# tex -> pdf ##################################################################

ifneq ($(PDFLATEX),)
%.pdf: %.tex $(source_files)
	@echo
	@echo ">>>>>>>>>>> latexing $(@:.pdf=)  <<<<<<<<<<<"
	@$(PDFLATEX) $(@:.pdf=) </dev/null
	@echo ">>>>>>>>>>> bibtexing $(@:.pdf=) <<<<<<<<<<<"
	@egrep "$(@:.pdf=.bbl)" $(@:.pdf=.log) >/dev/null && bibtex $(@:.pdf=) ; true
	@echo ">>>>>>>>>>> indexing $(@:.pdf=)  <<<<<<<<<<<"
	@egrep "Writing index file" $(@:.pdf=.log) | colrm 1 19 | xargs -n 1 makeindex ; true
	@echo ">>>>>>>>>>> latexing $(@:.pdf=)  <<<<<<<<<<<"
	@$(PDFLATEX) $(@:.pdf=) </dev/null
	@egrep $(latex_needs_rerun_pattern) $(@:.pdf=.log) && \
     echo ">>>>>>>>>>> latexing $(@:.pdf=)  <<<<<<<<<<<" && $(PDFLATEX) $(@:.pdf=) </dev/null; true
	@egrep $(latex_needs_rerun_pattern) $(@:.pdf=.log) && \
     echo ">>>>>>>>>>> latexing $(@:.pdf=)  <<<<<<<<<<<" && $(PDFLATEX) $(@:.pdf=) </dev/null; true
	@echo ">>>>>>>>>>> grepped error messages begin: $(@:.pdf=) <<<<<<<<<<<"
	@egrep $(latex_error_report_pattern)  $(@:.pdf=.log) | grep -v "Missing character:" ; true
	@echo ">>>>>>>>>>> grepped error messages end: $(@:.pdf=) <<<<<<<<<<<"
endif

# simple conversion ############################################################

%.pdf: %.ps
	ps2pdf $< $@

%.embedded.pdf: %.ps
	gs -q -dEmbedAllFonts=true -dNOPAUSE -dBATCH -sPAPERSIZE=$(papersize) \
        -dPDFSETTINGS=/prepress -sDEVICE=pdfwrite -sOutputFile=$@ -c save pop \
        -f $<

%.ps: %.dvi
	dvips -o $@ $<

%.eps: $.dvi
	dvips -E $< -o $@

# dia -> pdf ###################################################################

$(dia_pdf_include_files): %.pdf: %.dia
	dia -t pdf -e $@ $< 

# gnuplot -> ps, pdf ##########################################################

$(gnuplot_pdf_include_files): %.pdf: %.ps
	epstopdf $<
#	ps2pdf $< $@

$(gnuplot_ps_include_files): %.ps: %.gnuplot
	cd $(dir $@); gnuplot < $(notdir $<) > $(notdir $@)




